Latent Multi-group Membership Graph Model

We develop the Latent Multi-group Membership Graph (LMMG) model, a model of networks with rich node feature structure. In the LMMG model, each node belongs to multiple groups and each latent group models the occurrence of links as well as the node feature structure. The LMMG can be used to summarize the network structure, to predict links between the nodes, and to predict missing features of a node. We derive efficient inference and learning algorithms and evaluate the predictive performance of the LMMG on several social and document network datasets.

==> 020related.tex <==
Before describing our model, we begin by the survey of some related work.
% and then introduce the MAG model to help understanding.

\xhdr{Models of networks with node features}
%
A line of research has studied the network model considering node features.
Because of plentiful work on text documents,
there exist many document/coauthorship network models that incorporate the topic from documents.
%\textit{Nallapati et. al.}~\yrcite{nallapati08lda} blends 
For example, the Pairwise Link-LDA model (PL-LDA) nicely blends the Mixed-membership Stochastic Blockmodel and the Latent Dirichlent Allocation into one framework with regard to document network~\cite{nallapati08lda}.
%\textit{Chang \& Blei}~\cite{chang09rtm} proposes 
Another example includes the Relational Topic Model (RTM) which defines the relationships between documents on top of LDA topic model~\cite{chang09rtm}.
However, the node features of both models are limited to words which have the same distribution according to the topic,
whereas the node features in our model do not have such restriction.

\hide{
Also in the biology, there have been similar attempts 
%to deal with both network and node features 
to present a method for clustering genes
based on microarray expression data (node features) and a given gene network~\cite{shiga07gene}.
}
%\textit{Shiga et. al.}~\cite{shiga07gene} presents a method for clustering genes using microarray expression data (features) and a given gene network.

Historically, the above models have been however developed by smoothly turning focus to networks from long-lived text analysis research with vector form of data.
In contrast, the Exponential Random Graph Model (ERGM)~\cite{ergm} and the Multiplicative Attribute Graphs (MAG) model~\cite{mh12mag} have added a framework for node features on top of network model.
While ERGM pays more attention to the local network patterns, the MAG model considers the global network structure, similarly to our approach, so that it 
%Due to its origin, it can give rise to networks 
holds most real-world network properties such as small diameter~\cite{watts98smallworld}.
However, the MAG model is difficult to by itself determine proper combination of real-world node features associated with the network structure.
Our model resolves this issue by nicely connecting the global network structure to real-world node features via latent \topic s.


\xhdr{Collective classification}
%
In addition to network models with node features,
there have been attempts to exploit the network dependencies as well as node features for the node labeling task.
\textit{Collective Classification} is one of the methods to consider the network dependencies under the supervised setting~\cite{srl08ai}. 
For example, based on the assumption of homophily (more links between nodes with the same features), one can take the aggregate information of neighbor nodes as one feature of supervised learning.
%A lot of research has further studied this approach~\cite{TODO},
However, the attention has been paid more to the classification task than the generative model for node features and network links.
Moreover, this approach usually focuses only on the neighbors of a given node due to the homophily assumption,
while our model can capture more flexible global network structure,
% in terms of the MAG model.
%Since it is shown that the MAG model can capture more flexible structure 
including homophily (love of the same), heterophily (love of the different), and core-periphery (love of the core).
%we can utilize such various network structure which cannot be captured by collective classification.

%\xhdr{Network Model with Latent Topics}
%
%Network models defined by latent topics, groups or features have been already studied well in this literature.
%The examples of this line of work include the Mixed Membership Stochastic Block model (MMSB)~\cite{airoldi07blockmodel} and the Latent Dirichlet Allocation for Graphs (LDA-G)~\cite{henderson09glda}.
%Both models assume the latent group (topic) allocated by dirichlet distribution.
%MMSB defines the link probability between two nodes depending the groups that the two nodes are allocated to,
%whereas LDA-G determines the link probability based on the group which only the source node of a directed edge belongs to.
%However, the latent topics in the both models are fundamentally different from those in the \model .
%While the topics in MMSB and LDA-G are exclusive in a sense that each node is allocated to one topic at one link creation,
%in our model each node can independently belong to multiple \topic s. 
%}

\hide{
\xhdr{Multiplicative Attribute Graphs model}
%
Since we use the MAG model to generate network connections, here we explain it in more detail.
Assuming that a series of binary attributes for every node are appropriately given, 
the MAG model defines a \textit{link-affinity} associated with each attribute.
The link-affinity subject to an attribute means a tendency of linking between a pair of nodes,
where each of the pair has the corresponding value for the given attribute.
The link-affinity matrix is then defined as a table of every possible link-affinity with regard to the attribute.
As the node attributes are binary, each link-affinity matrix should be a 2 by 2 matrix.
Once link-affinity matrices are defined,
the MAG model determines the link probability between a pair of nodes
by multiplying the corresponding link-affinity values for all the attributes.

%\item Mutliplicative Attribute Graphs (MAG) model provides a way of connecting node attributes and network links~\cite{mh12mag}.
%\item However, the question of which real attributes have effects on the network connectivities has not been resolved~\cite{mh11magfit}.

Figure~\ref{fig:mag} visually explains the process of computing a link probability between node $i$ and $j$.
Given their attributes $F_{i}$ and $F_{j}$,
each attribute value for both nodes properly ``selects'' an entry in the corresponding link-affinity matrix
and the link probability $p_{ij}$ is then defined by the product of selected entry values.
Finally, the link between node $i$ and $j$ is generated by a coin-flip with probability $p_{ij}$.

As seen in the above process, the node attributes play a key role in network generation in the MAG model.
Again, the MAG model alone is, however, insufficient to explain which real-world node attributes are related to the network structure and how they are related.
Therefore, in the following section we present the framework of relating the MAG model to the real-world node features.
}


==> Makefile <==
RCSFLAGS= -l
MAIN=icml-maglda
TEXPARTS= \
	000abstract.tex		\
	010intro.tex		\
	020related.tex		\
	030model.tex		\
	040algorithm.tex	\
	050experiments.tex	\
	060conclusion.tex	\
	070appendix.tex

BIBPARTS= *.bib
LPR = pspr # or change to 'qpr -q ps3'
POSTSCRIPT= dvips -P cmz -t letter  #dvips -f
FIGPARTS = FIG

$(MAIN).ps: $(MAIN).dvi
	$(POSTSCRIPT) -o $(MAIN).ps $(MAIN).dvi
	ps2pdf $(MAIN).ps $(MAIN).pdf
:
try: $(MAIN).tex
	latex $(MAIN)

$(MAIN).dvi: $(MAIN).tex $(TEXPARTS) $(BIBPARTS)
	latex $(MAIN).tex
	bibtex $(MAIN)
	latex $(MAIN).tex
	latex $(MAIN).tex

print: $(MAIN).ps
	$(LPR) $(MAIN).ps

checkout:
	cvs checkout $(RCSFLAGS) $(MAIN).tex $(TEXPARTS)

checkin:
	cvs checkin $(RCSFLAGS) -f $(MAIN).tex $(TEXPARTS)

clean:
	\rm -f *.dvi $(MAIN).ps *.bbl *.aux *.log *.blg *.toc all.tar* uu *~ *.bak

spotless: clean
	\rm -f $(MAIN).ps

all.tar:
	tar cvfh all.tar makefile $(MAIN).tex $(TEXPARTS) $(BIBPARTS) \
	$(FIGPARTS) README

uu: all.tar
	gzip all.tar
	uuencode all.tar.gz all.tar.gz > uu

bundle.all: $(TEXPARTS) 
	bundle  README $(TEXPARTS) $(BIBPARTS) makefile > bundle.all

zip:
	cmd /C "pkzip $(MAIN).zip -P $(MAIN).pdf Makefile *.cls *.tex *.bib FIG/*.eps"

